Search for the Standard Model Higgs boson produced by vector-boson fusion in 8 TeV $pp$ collisions and decaying to bottom quarks with the ATLAS detector

A search with the ATLAS detector is presented for the Standard Model Higgs boson produced by vector-boson fusion and decaying to a pair of bottom quarks, using 20.2 ${fb}^{-1}$ of LHC proton-proton collision data at $\sqrt{s}$ = 8 TeV. The signal is searched for as a resonance in the invariant mass distribution of a pair of jets containing $b$-hadrons in vector-boson-fusion candidate events. The yield is measured to be $-0.8 \pm 2.3$ times the Standard Model cross-section for a Higgs boson mass of 125 GeV. The upper limit on the cross-section times the branching ratio is found to be 4.4 times the Standard Model cross-section at the 95% confidence level, consistent with the expected limit value of 5.4 (5.7) in the background-only (Standard Model production) hypothesis.

==> Sec_Auxiliary.tex <==




\begin{figure}[!h]
 \centering
 \includegraphics[width=0.65\textwidth]{figures/ws_root_pulls_125}
 \caption{
Impact of systematic uncertainties on the fitted signal-strength parameter, $\hat{\mu}$. 
The systematic uncertainties are listed in decreasing order of their impact on $\hat{\mu}$ 
on the vertical-axis. 
The boxes show the variations of $\hat{\mu}$, referring to the top horizontal-axis, when fixing the corresponding 
individual nuisance parameter $\theta$ to its post-fit value $\hat{\theta}$ modified upwards or downwards 
by its post-fit uncertainty, and repeating the fit. The hatched and open areas correspond to the upwards 
and downwards variations, respectively. The points, referring to the bottom horizontal-axis, show the 
deviations of a fitted nuisance parameter $\hat{\theta}$ from its nominal value $\theta_0$, expressed 
in terms of standard deviations with respect to its pre-fit uncertainty $\Delta\theta$. The associated 
error bars show the post-fit uncertainties of the nuisance parameters, relative to their pre-fit uncertainties.  
The jet energy scale uncertainty is decomposed into uncorrelated components; the labels from 14 to 15 refer to such components. 
Similarly, the background modelling uncertainty due to the choice of the fit function, for each BDT output category 
(referred to as Cat.I, Cat.II, Cat.III, and Cat.IV), is decomposed into uncorrelated components; the labels Var. 1 and Var. 2 
refer to such components. The uncertainties due to the $Z$ yield are both correlated among the categories, or specific for each category.  
The MC statistics enters both as a bin-by-bin systematic, and as the fraction of the resonant components in each category. 
The Higgs boson fraction in category IV is shown among the most relevant uncertainties. Finally, the MC signal 
modelling gives a contribution to the systematic uncertainties, as explained in the paper.}
 \label{fig:aux_cutbased}
\end{figure} 


==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2013
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

